SwiftSketch: A Diffusion Model for Image-to-Vector Sketch Generation

Recent advancements in large vision-language models have enabled highly expressive and diverse vector sketch generation. However, state-of-the-art methods rely on a time-consuming optimization process involving repeated feedback from a pretrained model to determine stroke placement. Consequently, despite producing impressive sketches, these methods are limited in practical applications. In this work, we introduce SwiftSketch, a diffusion model for image-conditioned vector sketch generation that can produce high-quality sketches in less than a second. SwiftSketch operates by progressively denoising stroke control points sampled from a Gaussian distribution. Its transformer-decoder architecture is designed to effectively handle the discrete nature of vector representation and capture the inherent global dependencies between strokes. To train SwiftSketch, we construct a synthetic dataset of image-sketch pairs, addressing the limitations of existing sketch datasets, which are often created by non-artists and lack professional quality. For generating these synthetic sketches, we introduce ControlSketch, a method that enhances SDS-based techniques by incorporating precise spatial control through a depth-aware ControlNet. We demonstrate that SwiftSketch generalizes across diverse concepts, efficiently producing sketches that combine high fidelity with a natural and visually appealing style.

==> tables/metrics.tex <==






\begin{table*}
\small
\setlength{\tabcolsep}{4pt}
\centering
\caption{Quantitative Comparison of Sketch Generation Methods. The scores for Top-1 and Top-3 CLIP recognition accuracy, MS-SSIM, and DreamSim are presented. Results are based on 6,000 random samples: 2,000 from our dataset's test set, 2,000 from unseen categories in our dataset, and 2,000 from the external SketchyCOCO dataset \cite{SketchyCOCO2020}. The best scores in each column are marked in bold.}\vspace{-0.2cm}
\begin{tabular}{l l c c c c c c c c c c c c} 
    \toprule
    & & \multicolumn{3}{c}{CLIP Top-1 $\uparrow$} & \multicolumn{3}{c}{CLIP Top-3 $\uparrow$}  & \multicolumn{3}{c}{MS-SSIM $\uparrow$} & \multicolumn{3}{c}{DreamSim $\downarrow$}  \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
    & Time & Seen & Unseen & Exter. & Seen & Unseen & Exter. & Seen & Unseen & Exter. & Seen & Unseen & Exter. \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-9}\cmidrule(lr){10-10}\cmidrule(lr){11-11}\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
    Human \shortcite{SketchyCOCO2020} & $-$ & $-$ & $-$ & $0.85$ & $-$ & $-$ & $0.93$ & $-$ & $-$ & \textcolor{black}{$0.16$} & $-$ & $-$ & \textcolor{black}{$0.66$} \\
    Chan \etal (Anime) \shortcite{Chan2022LearningTG} & $\approx$ 0.04 sec. & $0.94$  & \textcolor{black}{$\mathbf{0.99}$} & $0.87$ & \textcolor{black}{$\mathbf{0.99}$} & \textcolor{black}{$\mathbf{0.99}$} & $0.96$ & $0.79$ & $0.77$ & $0.45$ & \textcolor{black}{$\mathbf{0.32}$} & \textcolor{black}{$\mathbf{0.43}$} & \textcolor{black}{$\mathbf{0.45}$} \\
    Chan \etal (Contour) \shortcite{Chan2022LearningTG} & $\approx$ 0.04 sec. & $0.96$  & $0.92$ & $0.80$ & $0.98$ & $0.95$ & $0.91$ & $0.77$ & $0.73$ & $0.49$ &  $0.51$ & $0.59$ & $0.54$  \\
    InstantStyle \shortcite{Wang2024InstantStyleFL} & $\approx$ 1 min. & $0.97$ & \textcolor{black}{$\mathbf{0.99}$} & $-$  & \textcolor{black}{$\mathbf{0.99}$} & \textcolor{black}{$\mathbf{0.99}$} & $-$ & \textcolor{black}{$\mathbf{0.89}$} & \textcolor{black}{$\mathbf{0.90}$} & $-$ & $0.36$ & $0.44$ & $-$ \\
    Photo-Sketching \shortcite{Li2019PhotoSketchingIC} & $\approx$ 0.6 sec. & \textcolor{black}{$0.90$} & $0.81$ &  $0.65$ & \textcolor{black}{$0.95$} & $0.87$ & $0.78$ & $0.61$ & $0.55$ & $0.40$ & $0.58$ & $0.65$ & $0.63$ \\
    CLIPasso \shortcite{vinker2022clipasso} & $\approx$ 5 min. & \textcolor{black}{$\mathbf{0.98}$}  & $0.97$ & $0.88$ & $\mathbf{0.99}$ & $\mathbf{0.99}$ & $0.95$ & $0.65$ & $0.60$ & $0.52$ & $0.48$ & $0.57$ & $0.57$  \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-14}
    ControlSketch & $\approx$ 10 min. & $0.97$ & $0.97$ & \textcolor{black}{$\mathbf{0.91}$}  & \textcolor{black}{$\mathbf{0.99}$} & \textcolor{black}{$\mathbf{0.99}$} &  \textcolor{black}{$\mathbf{0.97}$} & $0.68$ & $0.63$ & $\mathbf{0.53}$ & $0.52$ & $0.59$  & $0.60$ \\
    SwiftSketch & $\approx$ 0.5 sec. & $0.95$ & \textcolor{black}{$0.70$} & \textcolor{black}{$0.56$} & $0.98$ & \textcolor{black}{$0.82$} &  $0.70$ & $0.62$ & $0.56$ & $0.47$ & $0.53$ & $0.66$  & $0.64$ \\
    
    \bottomrule
\end{tabular}
\label{tb:clip_metrics}
\end{table*}






    
    


==> tables/metrics_ablation.tex <==


    

    


\begin{table}
\small
\setlength{\tabcolsep}{2.5pt}
\addtolength{\belowcaptionskip}{-5pt}
\centering
\caption{Ablation Study. We systematically remove each component in our pipeline and retrain our network. Scores are computed on 4000 sketches in total: 2000 from seen categories and 2000 from unseen categories.} \vspace{-0.2cm}
\begin{tabular}{l c c c c c c c c c } 
    \toprule
    & \multicolumn{2}{c}{CLIP Top-1 $\uparrow$} & \multicolumn{2}{c}{CLIP Top-3 $\uparrow$}  & \multicolumn{2}{c}{MS-SSIM $\uparrow$} & \multicolumn{2}{c}{DreamSim $\downarrow$}  \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
    
     & Seen & Unseen  & Seen & Unseen & Seen & Unseen  & Seen & Unseen  \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-9}

    w/o LPIPS  & $0.88$ & $0.36$ & $0.94$ & $0.49$ & $0.58$ & $0.52$ & $0.58$ & $0.72$  \\
    w/o L1  & $0.03$ & $0.01$ & $0.06$ & $0.03$ & $0.24$ & $0.22$ & $0.80$ & $0.84$  \\
    w/o Sorting  & $0.93$ & $0.63$ & $0.97$ & $0.76$ & \textcolor{black}{$\mathbf{0.62}$} &  \textcolor{black}{$\mathbf{0.57}$}  & $0.55$ & $0.68$  \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-9}
    \makecell[l]{Full}  & $0.94$ & $0.61$ & $0.97$ & $0.73$ & \textcolor{black}{$\mathbf{0.62}$}  &  \textcolor{black}{$\mathbf{0.57}$}  & $0.54$ & $0.68$  \\
    
    +Refine  & \textcolor{black}{$\mathbf{0.95}$}  &  \textcolor{black}{$\mathbf{0.70}$}   & \textcolor{black}{$\mathbf{0.98}$}  &  \textcolor{black}{$\mathbf{0.82}$}  &  \textcolor{black}{$\mathbf{0.62}$}  & $0.56$  &  \textcolor{black}{$\mathbf{0.53}$}  & \textcolor{black}{$\mathbf{0.66}$}  \\
    
    \bottomrule
\end{tabular}
\label{tb:ablation_metrics}
\end{table}





==> tables/quali_all.tex <==
\begin{figure*}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    {\small
    \begin{tabular}{c |c c c c c |c c}
         \midrule
         & XDoG &  Chan et al. & Instant-Style  & Photo-Sketching & CLIPasso & ControlSketch  & SwiftSketch \\
        \midrule
        Time | \textcolor{orange}{\textbf{P}}/\textcolor{cyan}{\textbf{V}} &$\approx$ 0.1 sec. | \textcolor{orange}{\textbf{P}} & $\approx$ 0.04 sec. | \textcolor{orange}{\textbf{P}} & $\approx$ 1 min.| \textcolor{orange}{\textbf{P}} & $\approx 0.6 $ sec.| \textcolor{orange}{\textbf{P}} & $\approx 5$ min. | \textcolor{cyan}{\textbf{V}} & $\approx 10$ min. | \textcolor{cyan}{\textbf{V}} & $\approx 0.5 $ sec.| \textcolor{cyan}{\textbf{V}} \\
        \midrule
        \includegraphics[trim=4cm 1.8cm 4cm 2.5cm,clip,width=0.11\textwidth]{figs/comparisons/robot/input_robot_7311.jpg} &
        \includegraphics[trim=4cm 1.8cm 4cm 2.5cm,clip,width=0.11\textwidth]{figs/comparisons/robot/xdog_robot_7311.jpg} &
        \includegraphics[trim=1cm 0.45cm 1cm 0.6cm,clip,width=0.11\textwidth]{figs/comparisons/robot/robot_7311_informative-drawings.png} &
        \includegraphics[trim=4cm 1.9cm 4cm 2.1cm,clip,width=0.11\textwidth]{figs/comparisons/robot/robot_7311_InstantStyle-Plus.jpg} &
        \includegraphics[trim=1cm 0.45cm 1cm 0.6cm,clip,width=0.11\textwidth]{figs/comparisons/robot/robot_7311_PhotoSketch.png} &
        \includegraphics[trim=1.6cm 0.7cm 1.6cm 0.8cm,clip,width=0.11\textwidth]{figs/comparisons/robot/robot_7311_CLIPasso.png} &
        \includegraphics[trim=1.6cm 0.7cm 1.6cm 0.8cm,clip,width=0.11\textwidth]{figs/comparisons/robot/robot_7311_control_sketch.png}  &
        \includegraphics[trim=1.6cm 0.7cm 1.6cm 0.8cm,clip,width=0.11\textwidth]{figs/comparisons/robot/robot_7311_refine_swift_sketch.png} \\

        \includegraphics[trim=0 1.8cm 4cm 4cm,clip,width=0.11\textwidth]{figs/comparisons/horse/input_horse_61.jpg} &
        \includegraphics[trim=0 1.8cm 4cm 4cm,clip,width=0.11\textwidth]{figs/comparisons/horse/xdog_horse_61.jpg} &
        
        \includegraphics[trim=0 0.5cm 1cm 1cm,clip,width=0.11\textwidth]{figs/comparisons/horse/horse_61_informative-drawings.png} &
        \includegraphics[trim=0 1.8cm 4cm 4cm,clip,width=0.11\textwidth]{figs/comparisons/horse/horse_61_InstantStyle-Plus.jpg} 
        &
        \includegraphics[trim=0 0.5cm 1cm 1cm,clip,width=0.11\textwidth]{figs/comparisons/horse/horse_61_PhotoSketch.png} &
        \includegraphics[trim=0 0.9cm 1.7cm 1.6cm,clip,width=0.11\textwidth]{figs/comparisons/horse/horse_61_CLIPasso.png} &
        \includegraphics[trim=0 0.9cm 1.6cm 1.6cm,clip,width=0.11\textwidth]{figs/comparisons/horse/horse_61_control_sketch.png}  &
        \includegraphics[trim=0 0.9cm 1.6cm 1.6cm,clip,width=0.11\textwidth]{figs/comparisons/horse/horse_61_refine_swift_sketch.png} \\

        \includegraphics[trim=0 7cm 0 6cm,clip,width=0.11\textwidth]{figs/comparisons/squirrel/input_squirrel_22530.jpg} &
        \includegraphics[trim=0 7cm 0 6cm,clip,width=0.11\textwidth]{figs/comparisons/squirrel/xdog_squirrel_22530.jpg} &
        
        \includegraphics[trim=0 1.8cm 0 1.5cm,clip,width=0.11\textwidth]{figs/comparisons/squirrel/squirrel_22530_informative-drawings.png} &
        \includegraphics[trim=0 7cm 0 6cm,clip,width=0.11\textwidth]{figs/comparisons/squirrel/squirrel_22530_InstantStyle-Plus.jpg}         &
        \includegraphics[trim=0 1.8cm 0 1.35cm,clip,width=0.11\textwidth]{figs/comparisons/squirrel/squirrel_22530_PhotoSketch.png} &
        \includegraphics[trim=0 3.5cm 0 2.1cm,clip,width=0.11\textwidth]{figs/comparisons/squirrel/squirrel_22530_CLIPasso.png} &
        \includegraphics[trim=0 3.5cm 0 2.1cm,clip,width=0.11\textwidth]{figs/comparisons/squirrel/squirrel_22530_control_sketch.png}  &
        \includegraphics[trim=0 3.5cm 0 2.1cm,clip,width=0.11\textwidth]{figs/comparisons/squirrel/squirrel_22530_refine_swift_sketch.png}  \\

    
    \end{tabular}
    }
    \vspace{-0.4cm}
    \caption{Qualitative Comparison. Input images are shown on the left, with the time required to produce a single sketch and whether the sketches are in \textcolor{orange}{\textbf{P}}ixel or \textcolor{cyan}{\textbf{V}}ector format indicated at the top. From left to right, the sketches are generated using XDoG \shortcite{Winnemller2011XDoGAI}, PhotoSketching \shortcite{Li2019PhotoSketchingIC}, Chan et al. \shortcite{Chan2022LearningTG} (in anime style), InstantStyle \shortcite{Wang2024InstantStyleFL}, and CLIPasso \shortcite{vinker2022clipasso}. On the right are the resulting sketches from our proposed methods, ControlSketch and SwiftSketch.}
    \label{fig:comparison}
\end{figure*}

